Saga: A Platform for Continuous Construction and Serving of Knowledge At Scale

We introduce Saga, a next-generation knowledge construction and serving platform for powering knowledge-based applications at industrial scale. Saga follows a hybrid batch-incremental design to continuously integrate billions of facts about real-world entities and construct a central knowledge graph that supports multiple production use cases with diverse requirements around data freshness, accuracy, and availability. In this paper, we discuss the unique challenges associated with knowledge graph construction at industrial scale, and review the main components of Saga and how they address these challenges. Finally, we share lessons-learned from a wide array of production use cases powered by Saga.

==> sections_sigmod/lessons.tex <==
%!TEX root = ../siribase_paper.tex

\section{Lessons Learned}\label{sec:lessons}

==> sections_sigmod/selfserve.tex <==
%!TEX root = ../siribase_paper.tex
\section{Self-Serve Knowledge Onboarding}\label{sec:selfserve}
\ihab{Mohamed}

\subsection{Mapping Tooling}
\subsection{Extensible Adaptors and Linkers}
Config-driven 

==> sections_sigmod/system.tex <==
%!TEX root = ../siribase_paper.tex

\section{System Overview}\label{sec:system}

\subsection{Incremental Open-Domain Record Linkage}\label{sec:record_linkage}

\subsection{Data Governance-aware Data Fusion}\label{sec:fusion}

\subsection{Graph Query and View Engine}\label{sec:graph_engine}

\subsection{Knowledge Graph Profiling and Cleaning}\label{sec:profiling}

\subsection{On-Demand Knowledge Completion and Verification}\label{sec:complete_verify}

\subsection{Run-time Graph Serving}\label{sec:serve}
